Scalable Automated Verification for Cyber-Physical Systems in Isabelle/HOL

We formally introduce IsaVODEs (Isabelle verification with Ordinary Differential Equations), a framework for the verification of cyber-physical systems. We describe the semantic foundations of the framework's formalisation in the Isabelle/HOL proof assistant. A user-friendly language specification based on a robust state model makes our framework flexible and adaptable to various engineering workflows. New additions to the framework increase both its expressivity and proof automation. Specifically, formalisations related to forward diamond correctness specifications, certification of unique solutions to ordinary differential equations (ODEs) as flows, and invariant reasoning for systems of ODEs contribute to the framework's scalability and usability. Various examples and an evaluation validate the effectiveness of our framework.

==> sections/cas.tex <==
%%%%%%%%%%% COMPUTER ALGEBRA %%%%%%%%%%%%
\section{Solutions from Computer Algebra Systems}\label{sec:cas}
% TODO: distil section 7.3 into a couple of paragraphs
% TODO: merge 7.1 and 7.2

In this section we describe our approach to integrating SageMath and the Wolfram Engine, two Computer Algebra Systems (CASs), into Isabelle/HOL with the objective of supplying solutions to given SODEs. The user can make use of the integration via the  \isakwmaj{\textbf{find{\isacharunderscore}local{\isacharunderscore}flow}} command, which supplies a solution to the first SODE it finds within the current subgoal.

Below, we show an application of our integration and its corresponding output in Isabelle. Users can click the greyed-out area to automatically insert the suggestion. 

\begin{isabellebody}\isanewline
\isacommand{lemma}\ \isamarkupfalse%
local{\isacharunderscore}flow{\isacharunderscore}example{\isacharcolon}\isanewline
\ \ {\isachardoublequoteopen}\isactrlbold {\isacharbraceleft}{\kern0pt}x\ {\isachargreater}{\kern0pt}\ {\isadigit{0}}\isactrlbold {\isacharbraceright}{\kern0pt}\ x\ {\isacharcolon}{\isacharcolon}{\isacharequal}\ {\isadigit{1}}{\isacharsemicolon}\ {\isacharbraceleft}x{\isasymacute}\ {\isacharequal}\ {\isadigit{1}}{\isacharbraceright} \isactrlbold {\isacharbraceleft}{\kern0pt}x {\isachargreater}{\kern0pt}\ {\isadigit{1}}\isactrlbold {\isacharbraceright}{\kern0pt}{\isachardoublequoteclose}\isanewline
\ \ \isakwmaj{find{\isacharunderscore}local{\isacharunderscore}flow}\isanewline
\texttt{Output}:\isanewline
\ \ \texttt{Calling Wolfram...}\isanewline
\ \ {\isasymlambda}t{\isachardot}\ {\isacharbrackleft}x\ {\isasymleadsto}\ t\ {\isacharplus}\ {\isachardollar}x{\isacharbrackright}\isanewline
\ \ \texttt{try this:}\ {\setlength{\fboxsep}{0.1pt}\colorbox{lightgray}{apply (wlp{\isacharunderscore}solve {\isachardoublequoteopen}{\isasymlambda}t{\isachardot}\ {\isacharbrackleft}x\ {\isasymleadsto}\ t\ {\isacharplus}\ {\isachardollar}x{\isacharbrackright}{\isachardoublequoteclose})}}
\isanewline
\end{isabellebody}
\noindent Our integration follows the following steps in order to produce a solution:

\begin{enumerate}
    \item Retrieve an Isabelle term describing the SODEs.
    \item Convert the term into an intermediate representation.
    \item Use one of the CAS backends to solve the SODE.
    \item Convert the solution to an Isabelle term.
    \item Certify the solution using the \texttt{wlp\_solve} Isabelle tactic.
\end{enumerate}


\subsection{Intermediate representation}

\noindent In order to have an extensible and modular interface, we implement the below intermediate datatype for representing ODEs and their solutions, and procedures for translating back and forth between Isabelle and our intermediate representation. This allows us capture the structure of the ODEs without the added overhead of Isabelle syntax, and gives us a unified interface between Isabelle and any CAS integrations.

%\begin{minted}{SML}
\begin{alltt}
datatype AExp = NConst of string | UOp of string * AExp |
            BOp of string * AExp * AExp | NNat of int | NInt of int |
            NReal of real | CVar of string | SVar of string | IVar
\end{alltt}
%\end{minted}

\texttt{NConst} represents numeric constants, e.g. $e$ or $\pi$; \texttt{UOp} is for unary operations, \texttt{BOp} is for binary operations, \texttt{NNat} for naturals, \texttt{NInt} for integers and \texttt{NReal} for reals. We have three characterisations of variables: \texttt{CVar} are arbitrary but fixed variables, \texttt{SVar} are mutable (state) variables, and \texttt{IVar} represents the independent variable of our system, usually time.

Converting back and forth between Isabelle terms and the AExp datatype consists of recursing through the structure of the term, using a lookup table to translate each constructor. We implement two ways of representing SODEs in Isabelle: tuples and substitutions.

\subsection{CAS Integrations}

Integrating a CAS into our workflow generally consists of three separate components: translating from the intermediate representation to the CAS input format, interfacing with the CAS in order to obtain a solution, and converting the solution back into the required format.

\paragraph{Wolfram Engine}
The Wolfram Engine is the CAS behind WolframAlpha and Mathematica~\cite{wolfram_engine}. It is one of the leading CASs on the market, with powerful features for solving differential equations, amongst many other applications.

The basic building block for this integration is a representation of Wolfram expressions as an ML datatype. In the Wolfram language, everything is an expression, so this is sufficient for a complete interface. We represent expressions as follows:

\begin{alltt}
\textbf{datatype} expr = Int \textbf{of} int
              | Real \textbf{of} real
              | Id  \textbf{of} string
              | Fun \textbf{of} string * expr list
              | CurryFun \textbf{of} string * expr list list
\end{alltt}

\texttt{Real} and \texttt{Int} represent real and integer numbers respectively, Id are identifiers, and Fun represents functions with only one list of arguments, which are distinguished from curried functions CurryFun with multiple sets of arguments.

Our approach for translation from \texttt{AExp} to \texttt{expr} is the following:
\begin{enumerate}
    \item Generate an alphabetically ordered variable mapping to avoid name clashes and ease solution reconstruction.
    \item Traverse the expression tree and translate each term to Wolfram.
    \item Wrap in the Wolfram DSolve function, supplying the state and independent variables along with our ODE. 
\end{enumerate}

Once we have a well-formed Wolfram expression, we use the wolframscript command-line interface to obtain a solution in the form of a list of Wolfram \texttt{Rule} expressions, which are isomorphic to our substitutions. We can parse the result back into the \texttt{expr} type, and translate this into the \texttt{AExp} type using a translation table for function names and the variable name mapping we constructed.

\paragraph{SageMath}
SageMath~\cite{sagemath} is an open-source competitor to the Wolfram Engine. It is accessed via calls to a Python API. It integrates several open-source CASs to provide its functionality, choosing in each case the best implementation for a particular symbolic computation. This makes SageMath an ideal target for integration with Isabelle.

The translation process is similar to that of our Wolfram Engine integration, but we also apply some preprocessing to the SODEs in order to make the solving more efficient. Because the CASs integrated with SageMath are better at solving smaller SODEs, we can improve their performance by rewriting the following kinds of SODEs:

\begin{enumerate}
\item SODEs formed from a higher order ODE, where an extra variable has been introduced in order to make all derivatives first order, can be recast into their higher-order form. For example, the SODE \(x' = 2x+y, y'=x\) can be rewritten as \(x'' = 2x + x'\).  
\item Independent components of an SODE can be solved independently by the CAS. For example, in the SODE \(x' = x, t' = 1\), x and t are independent and so they can be solved independently.
\end{enumerate}

==> sections/oldcas.tex <==
\subsection{Certification}
\cpin{Complete narrative on the CAS pipeline.}

In this section we describe how SODE solutions can be certified using our \verb|ode_cert| proof tactic. We assume a SODE of the form $\dot{x}~t = f~t~(x~t)$, described by a function $f : \real \to \real^n \to \real^n$, which gives a vector of derivatives for each continuous variable at time $t$ and current state $x~t$. A candidate solution to this SODE is a function $x : \real \to \real^n$, which can potentially have a restricted domain $T \subseteq \real$ and range $D \subseteq \real^n$. For example, consider the following SODE:
\begin{example} \label{ex:SODE} $(\dot{x}(t), \dot{y}(t), \dot{z}(t)) = (t, x(t), 1)$
\end{example}
It has three continuous variables, and can be represented with the function $g \defs (\lambda\,t~(x, y, z).\, (t, x, 1)$ whose type is $\real \to \real^3 \to \real^3$. Its representation in Isabelle is shown in Figure~\ref{fig:repr}, where a name is introduced for it by an abbreviation.



The goal of the \texttt{ode\_cert} tactic, then, is to prove conjectures of the form $$x \mathop{\skey{solves-ode}} f~T~D$$ which specifies that $x$ is indeed a solution to $f$, and is defined within the \textsf{HOL-ODE} package~\cite{Immler12}. It requires that we solve the following two predicates:
$$(\forall t \in T.\, (x \mathop{\skey{has-vector-derivative}} ~(f~t~(x~t))~ (\skey{at}~t~\skey{within}~T))) ~\text{and}~ x \in T \to D$$
We need to show that at every $t$ in the domain, the derivative of $x$ matches the one predicted by $f$, and that $x$ has the correct domain and range. The predicate $\skey{has-vector-derivative}$ is defined within the \textsf{HOL-Analysis} package~\cite{Harrison2005-Euclidean}, which also provides a large library of differentiation theorems. For brevity, we use the syntax $\hvderiv{f}{f'}{t}{T}$ to mean $(f \mathop{\skey{has-vector-derivative}} f') (\skey{at}~t~\skey{within}~T)$.

\begin{theorem}[Derivative Introduction Theorems] \label{thm:der-intro} $ $%

\vspace{2ex}

\centering
\begin{tabular}{cccc}

\AxiomC{---}
\RightLabel{\labelthis{rule:a}{a}}
\UnaryInfC{$\hvderiv{(\lambda x.\, c)}{0}{t}{T}$}
\DisplayProof
~~
\AxiomC{---}
\RightLabel{\labelthis{rule:b}{b}}
\UnaryInfC{$\hvderiv{(\lambda x.\, x)}{1}{t}{T}$}
\DisplayProof

\\[4ex]
\AxiomC{$\hvderiv{f}{f'}{t}{T}$}
\AxiomC{$\hvderiv{g}{g'}{t}{T}$}
\RightLabel{\labelthis{rule:c}{c}}
\BinaryInfC{$\hvderiv{(\lambda x. (f~x, g~x))}{(f', g')}{t}{T}$}
\DisplayProof
\qquad
\AxiomC{$\hvderiv{f}{f'}{t}{T}$}
\AxiomC{$\hvderiv{g}{g'}{t}{T}$}
\RightLabel{\labelthis{rule:d}{d}}
\BinaryInfC{$\hvderiv{(\lambda x. f~x + g~x)}{f'+ g'}{t}{T}$}
\DisplayProof
\\[4ex]
\AxiomC{$\hvderiv{f}{f'}{t}{T}$}
\RightLabel{\labelthis{rule:e}{e}}
\UnaryInfC{$\hvderiv{(\lambda x. \sin(f~x))}{(f' \cdot \cos(f~t)))}{t}{T}$}
\DisplayProof
\\[4ex]
\AxiomC{$\hvderiv{f}{f'}{t}{T}$}
\AxiomC{$f~t > 0$}
\RightLabel{\labelthis{rule:f}{f}}
\BinaryInfC{$\hvderiv{(\lambda x. \sqrt{f~x})}{(f' \cdot 1 / (2 \cdot \sqrt{f~t}))}{t}{T}$}
\DisplayProof
\\[4ex]
\AxiomC{$\hvderiv{f}{f'}{t}{T}$}
\AxiomC{$\hvderiv{g}{g'}{t}{T}$}
\AxiomC{$g~t \neq 0$}
\RightLabel{\labelthis{rule:g}{g}}
\TrinaryInfC{$\hvderiv{(\lambda x. f~x / g~x)}{(- f~t \cdot (1 / (g~t) \cdot g' \cdot 1 / (g~t)) + f' / g~t))}{t}{T}$}
\DisplayProof
\end{tabular}
\end{theorem}
%
These are standard laws, but in a deductive rather than equational form. A constant function $\lambda x.\, c$ has derivative $0$~\eqref{rule:a}, and the identity function $\lambda x. \, x$ has derivative $1$~\eqref{rule:b}. If a derivative is composed of a pair $(f', g')$ then it can be decomposed into two derivative proofs~\eqref{rule:c}. This law is particularly useful for decomposing a SODE into its component ODEs. A function composed of two summed components can similarly be composed~\eqref{rule:d}. The derivative of $\sin$ is $\cos$~\eqref{rule:e}. The remaining two rules are for square root~\eqref{rule:f} and division~\eqref{rule:g}. They both have additional provisos to avoid undefinedness. Square root $\sqrt{x}$ can be differentiated only when $x > 0$. Similarly, a division requires that the denominator is non-zero, hence the extra proviso.

The strategy employed by \texttt{ode\_cert} is as follows:

\begin{nonformat-algorithm}[SODE Certification Method] $ $%

\begin{enumerate}
    \item Decompose a SODE in $n$ variables to $n$ subgoals of the form $\hvderiv{f_i}{f_i'}{t}{T}$ for $1 \le i \le n$ \label{it:step1};
    \item Replace every such goal with two goals: $\hvderiv{f_i}{X_i}{t}{T}$ and $X_i = f_i'$ using a fresh meta-variable $X_i$. The latter goal is used to prove equivalence between the expected and actual derivative in $f'$;
    \item For each remaining derivative goal, recursively apply the derivative introduction laws (Theorem~\ref{thm:der-intro}). If any derivative goals remain, the method fails;
    \item The remaining subgoals are equalities and inequalities in the real variables. Attempt to discharge them all using real arithmetic and field laws using the simplifier tactic for recursive equational rewriting.
    \item If no goals remain, the ODE is certified.
\end{enumerate}
\end{nonformat-algorithm}
%
We exemplify this method with Example~\ref{ex:SODE}, using $f \defs (\lambda t~(x, y, z). (t, x, 1)$. A proposed solution is $x \defs (\lambda t. (t^2 / 2 + x_0, t^3 / 6 + x_0 \cdot t + y_0, z_0 + t))$, where $x_0, y_0, z_0$ are integration constants, or initial values for variables. We form the goal $x \mathop{\skey{solves-ode}} f~\real~\real^3$ and execute \texttt{ode\_cert}. The domain and range constraints are trivial in this case. Following step~\eqref{it:step1}, we obtain 3 subgoals: 

\begin{enumerate}
    \item $\hvderiv{(\lambda t.\, t^2 / 2 + x_0)}{t}{t}{T}$;
    \item $\hvderiv{(\lambda t.\, t^3 / 6 + x_0 \cdot t + y_0)}{x}{t}{T}$;
    \item $\hvderiv{(\lambda t.\, z_0 + t)}{1}{t}{T}$
\end{enumerate}
%
We focus on the second subgoal. Having applied the derivative introduction laws, we receive two proof obligations. The first is $6 \neq 0$, which is required since $6$ is the denominator in a division, and is trivial. The second is the following equality:
$$- (t^3) \cdot (1/6 \cdot 0 \cdot 1/6) + 3 \cdot 1 \cdot t^{3-1} / 6 + (x_0 \cdot 1 + 0 \cdot t) + 0 = t^2 / 2 + x_0$$
%
Though seemingly complex, it simplifies to give the desired result, since all but one of the summands reduce to $0$. This, and more complex goals, can be solved using the built-in simplification sets \texttt{algebra\_simps} and \texttt{field\_simps}. The other two derivative subgoals similarly reduce, and so the solution is certified.

% LINK TEXT: The CAS integration complements our verification workflow. In the next section we apply this and our other methods to a number of examples for the purposes of evaluation.


==> sections/shallow-expr.tex <==
%%%% SHALLOW EXPRESSIONS %%%%
\section{Shallow Expressions Component} 

\jhin{What have we added to the shallow expressions?}
\sfin{Tactic support: expr-simp, expr-auto, subst-eval}

Next we present our new shallow expression component to support the
intuitive expression syntax often used in programming languages and
verification approaches semantically. We model expressions as
functions $\src\rightarrow \view$ in Isabelle's own expression syntax,
which is processed entirely in its meta-language (ML). We aim to
suppress, e.g., $\lambda$-binders that typically pollute naive shallow
expressions ($\lambda \skey{s}.\, \lget_x~\skey{s} + \lget_y~\skey{s}$
versus $x + y$). Isabelle's syntax translations allow relating
syntactic and semantic representations, and ultimately designing
interfaces to modelling languages such as Modelica and Matlab.
%
%\vspace{-\baselineskip}
%\subsubsection{Syntax translation.}
%
%Isabelle implements a multi-stage syntax pipeline. Unicode strings are parsed
%and transformed into ``pre-terms''~\cite{Kuncar2019-IsabelleFoundation}:
%elements of the ML \texttt{term} type containing syntactic constants. These must
%be mapped to previously defined semantic constants by syntax translations,
%before they can be checked and certified in the Isabelle kernel. Printing
%reverses this pipeline, mapping terms to strings. The pipeline supports a host
%of syntactic constructions.
%
%We reuse this pipeline with small modifications for our bidirectional
%expression transformation, including pretty printing. We subject
%pre-terms to a lifting process, which replaces their free variables
%and constants, and inserts store variables ($\skey{s}$) and
%$\lambda$-binders. Its implementation uses the syntactic annotation
%$\ebrack{t}$ to lift the syntactic term $t$ to a semantic expression
%in the syntax translation rules
%%
%$$\begin{array}{ccc}
%  \ebrack{t} \syneq [\ebracku{t}]_{\skey{e}},  &\quad \ebracku{x} \syneq
%          \begin{cases}
%            \lambda \skey{s}.\, \lget_x~\skey{s} & \text{if } x \text{ is a lens},\\
%            \lambda \skey{s}.\, x & \text{otherwise},
%          \end{cases} &\quad \ebracku{f~t} \syneq \lambda \skey{s}.\, f~(\ebracku{t}~\skey{s}),
%  \end{array}$$
%%
%  where $p \syneq q$ means that pre-term $p$ is translated to term
%  $q$, and $q$ printed as $p$. Moreover, $[-]_{\skey{e}}$ is a
%  constant that marks lifted expressions that are embedded in
%  terms. The pretty printer can then recognise a lifted term and print
%  it. \hfill\isalink{https://github.com/isabelle-utp/Shallow-Expressions/blob/bddbf31a67859011c81e16ad3d6723d66ed9591e/Expressions.thy\#L58}
%
%  Intuitively, $\ebrack{t}$ is processed as follows. The syntax
%  processor first parses a pre-term from string $t$. Then our parse
%  translation traverses its syntax tree. Whenever it encounters a free
%  variable $x$, the type system determines from the context whether it
%  is a lens, in which case a $\lget_x$ is inserted. Otherwise it is
%  left unchanged as a logical variable. Function applications are left
%  unchanged by $\rightleftharpoons$, except for expression constructs
%  like $e[v/x]$.  For program variables $x$ and $y$ and logical
%  variable $z$, e.g.,
%  $\ebrack{(x + y)^2 / z} \rightleftharpoons [\lambda \skey{s}.\,
%  (\lget_x~\skey{s} + \lget_y~\skey{s})^2 / z]_{\skey{e}}$. Once an
%  expression has been processed, the resulting $\lambda$-term is
%  enclosed in $[-]_{\skey{e}}$.
%
%  In assignments $x := e$ and substitutions $[x \smapsto e]$, $e$ is
%  lifted automatically without user annotations. We can also lift
%correctness specifications and allow intuitive parsing of assertions:
%$\hoaretriple{P}{\prog}{Q} \syneq \ebrack{P} \le \wlp\, \prog\,
%\ebrack{Q}$. \hfill\isalink{https://github.com/isabelle-utp/Hybrid-Verification/blob/7baedd092dff0182336ef0bb6251fd8beff6a1cc/HS_Lens_Spartan.thy\#L67}
%
%\vspace{-\baselineskip}
%\subsubsection{Substitution.}  
%
%Though our expressions are functions, we can mimic syntactic
%evaluation of substitutions using the rule
%$\ebrack{\lambda \skey{s}.\, e(\skey{s})}[v/x]
%= \ebrack{\lambda \skey{s}.\, e(\lput_x~(v~s)~\skey{s})}$. This pushes
%the substitution through the expression marker, by applying an update
%to the store. This rule preserves the lifted syntax, e.g.  $((x + y)^2
%/ c)_e [2 \cdot x / y] $ simplifies to $((3 \cdot x)^2 / c)_e$. We can
%also use substitutions to determine whether a variable is used:
%$(x \unrest e) \Leftrightarrow \forall v.\, (e[v/x]) = e$, meaning $e$ does
%not depend on $x$ if substituting any value $v$ for $x$ leaves $e$
%(\S\ref{sec:hyb-store}), e.g. $\ebrack{5}[v/x] = \ebrack{5}$,
%and thus $x\unrest 5$. Checking $\unrest$ is usually automatic. More
%generally, lenses allow simulating many standard syntactic
%manipulations semantically to support
%VCG. \hfill\isalink{https://github.com/isabelle-utp/Shallow-Expressions/blob/bddbf31a67859011c81e16ad3d6723d66ed9591e/Substitutions.thy\#L247}

%With Isabelle's syntax translations, we can specify \skey{g-orbital-on}
%naturally as
%$\{x_1' = e_1, \cdots, x_n' = e_n ~|~ G \mathop{\,\skey{on}\,} U\,V\,
%\mathop{\,@\,} t_0\},$ where each $x_i$ is a summand of the lens
%$\{x_1, \cdots, x_n\}$. We use this notation in all our examples of
%\S\ref{sec:case-studies}.  Users can thus declare the ODEs in
%evolution commands coordinate-wise with lifted expressions $e_i$
%ranging over $\mathcal{S}$. The other parameters $G$, $U$, $V$ and
%$t_0$ can be omitted, which defaults them to constantly
%\texttt{true}, $\{t.\ t\geq 0\}$, $\csrc$ and $0$, respectively. We can 
%collapse further to $(x_1', \cdots, x_n') = (e_1, \cdots, e_n)$ or 
%$\vec{x}' = \vec{e}$,

==> sections/vcg.tex <==
%%%%%%%%%%%%% VCG ADDITIONS %%%%%%%%%%%%%
%\section{Verification Condition Generation}\label{sec:vcg}













